Implicit Integration for Articulated Bodies with Contact via the Nonconvex Maximal Dissipation Principle

We present non-convex maximal dissipation principle (NMDP), a time integration scheme for articulated bodies with simultaneous contacts. Our scheme resolves contact forces via the maximal dissipation principle (MDP). Prior MDP solvers compute contact forces via convex programming by assuming linearized dynamics integrated using the forward multistep scheme. Instead, we consider the coupled system of nonlinear Newton-Euler dynamics and MDP, which is time-integrated using the backward integration scheme. We show that the coupled system of equations can be solved efficiently using the projected gradient method with guaranteed convergence. We evaluate our method by predicting several locomotion trajectories for a quadruped robot. The results show that our NMDP scheme has several desirable properties including: (1) generalization to novel contact models; (2) superior stability under large timestep sizes; (3) consistent trajectory generation under varying timestep sizes.

==> ZOANA.tex <==
\section{Convergence Analysis Of ZO-PGM}
\begin{theorem}
There exists an $\alpha_7$ such that \prettyref{alg:ZOPGM} will generate a second order convergent sequence $\{K(\theta^k),w^k\}$ for all $\alpha\leq\alpha_7$.
\end{theorem}

==> teaser.tex <==
\begin{figure}[ht]
\centering
\scalebox{0.8}{
\begin{tikzpicture}[scale=1, auto]
\matrix[ampersand replacement=\&, row sep=0.5cm, column sep=0.4cm] {
\node[block] (G) {\textcolor{red}{Linearize} $G_\alpha(\theta,\theta_{-},\theta_{--},w)$}; \&
\node[block] (V) {Wrench Space $v_x($\textcolor{red}{$\theta_{-}$}$)$}; \\
\node[block] (T) {Robot Pose $\theta$}; \&
\node[block] (W) {Contact force $w$}; \\
};
\draw [arrow] (G) -- (V);
\draw [arrow] (V) -- (W);
\draw [arrow] (W) -- (T);
%\node[above,font=\large\bfseries] at ($(current bounding box.south west)+(0.3,0.)$) {(a)};
\end{tikzpicture}}
\caption{\label{fig:illusa} \small{We define $G_\alpha$ as the articulated body's governing equations of motion, formulated either as Newton-Euler's equation or as Position-Based Dynamics (PBD). Conventional MDP solvers first linearize dynamics and then solve MDP via quadratic programming (QP).}}
\vspace{-10px}
\end{figure}
\begin{figure}[ht]
\centering
\scalebox{0.8}{
\begin{tikzpicture}[scale=1, auto]
\matrix[ampersand replacement=\&, row sep=0.5cm, column sep=0.4cm] {
\node[block] (G) {\textcolor{red}{Nonlinear} $G_\alpha(\theta,\theta_{-},\theta_{--},w)$}; \&
\node[block] (V) {Wrench Space $v_x($\textcolor{red}{$\theta$}$)$}; \\
\node[block] (T) {Robot Pose $\theta$}; \&
\node[block] (W) {Contact force $w$}; \\
};
\draw [arrow] (G) -- (V);
\draw [arrow] (V) -- (W);
\draw [arrow] (W) -- (T);
\draw [arrow,color=red] (T) -- (G);
%\node[above,font=\large\bfseries] at ($(current bounding box.south west)+(0.3,0.)$) {(b)};
\end{tikzpicture}}
\caption{\label{fig:illusb} \small{We consider the three components (robot pose $\theta$ update, convex wrench space $v_x(\theta)$ update, and contact force $w$ update) as a coupled system of nonlinear equations.}} %\textcolor{red}{Again, this is not a very compelling figure. The symbols and block diagram are not meaningful. Few people use PBD, so this can be misleading.}}} %\textcolor{red}{Can you pick out a "star figure" to place here? E.g., frames from a simulation with large time steps using your method vs standard NE-MDP?}
\vspace{-10px}
\end{figure}
